Some Statistical and Data Challenges When Building Early-Stage Digital Experimentation and Measurement Capabilities

Digital experimentation and measurement (DEM) capabilities -- the knowledge and tools necessary to run experiments with digital products, services, or experiences and measure their impact -- are fast becoming part of the standard toolkit of digital/data-driven organisations in guiding business decisions. Many large technology companies report having mature DEM capabilities, and several businesses have been established purely to manage experiments for others. Given the growing evidence that data-driven organisations tend to outperform their non-data-driven counterparts, there has never been a greater need for organisations to build/acquire DEM capabilities to thrive in the current digital era. This thesis presents several novel approaches to statistical and data challenges for organisations building DEM capabilities. We focus on the fundamentals associated with building DEM capabilities, which lead to a richer understanding of the underlying assumptions and thus enable us to develop more appropriate capabilities. We address why one should engage in DEM by quantifying the benefits and risks of acquiring DEM capabilities. This is done using a ranking under lower uncertainty model, enabling one to construct a business case. We also examine what ingredients are necessary to run digital experiments. In addition to clarifying the existing literature around statistical tests, datasets, and methods in experimental design and causal inference, we construct an additional dataset and detailed case studies on applying state-of-the-art methods. Finally, we investigate when a digital experiment design would outperform another, leading to an evaluation framework that compares competing designs' data efficiency.

==> challenges/challenges.tex <==
\chapter{Miscellaneous Expositions}

\section{Examples Where Digital Experimentation Differs From Other Fields}

In Chapter~\ref{chap:introduction}, we noted that digital experimentation brings different opportunities and challenges than experiments in other fields, e.g., agriculture, medicine, and economics. We provide a few examples in this section.

\paragraph{Systems can be scaled to cover many hypotheses and experimental units} Modern digital systems enable experimenters to set up many experiments in parallel, as well as interact and collect responses from thousands or even millions of experiment participants. All of these can happen at a fraction of the time and resource cost compared to offline, manually run experiments that were common decades ago. While they enable experimenters to try out many more ideas within a shorter duration, they also increase the risk of incurring different biases during experiment analysis. These include multiple comparisons (i.e., the more you look for, the more you see), seasonality (i.e., short-term experiment results not generalising to long-term experiment participant behaviour), and interaction between experiments (i.e., two ideas working well in isolation may be unsuccessful if combined).

\paragraph{Improvements having a small yet commercially significant effect}
Many successful digital experiments only improve on a decision metric by a fraction of a percent~\cite{kohavi2014sevenrules}, a result of the doctrine of ``marginal gains in quick cycles'' followed by many digital technology organisations. This is in stark contrast with, e.g., medical trials, where a drug or procedure that leads to a five or ten percentage point change in a decision metric (e.g., hospitalisation rate) may be considered as having a small effect.
Nonetheless, it remains critical to differentiate such a small effect from pure randomness, as a vast user base can translate it to millions of pounds worth of revenue and profit~\cite{xie16improving}. 

The setting can sometimes lead to a paradox where having more users reduces the treatment effect size required to achieve a practical impact, which requires even more users to distinguish the signal from the noise. Consider a team tasked to bring in an extra 1000 money units in revenue by increasing the proportion of website visitors who purchase (\emph{purchase proportion} hereafter), a figure considered practical to justify any development effort. If the website sees \numprint{100000} visitors and each visitor that makes a purchase spends one money unit, the team would need to drive \numprint{1000} extra visitors to purchase, i.e., a one percentage point increase in purchase proportion compared to the baseline. 

Now, suppose the website sees double the number of visitors (i.e., \numprint{200000}). In that case, the team will still need to drive \numprint{1000} extra visitors to purchase to bring in the same extra revenue, though these \numprint{1000} visitors only translate to half a percentage point increase in purchase proportion. A (null hypothesis) statistical test on whether the team's work has increased the purchase proportion will see the (relative) effect size to detect halved from the first to the second scenario. In the absence of other statistical tricks, this generally requires four times the number of samples to ``see'' the effect (more technically, achieve the same \emph{test power})~\cite{mcdonald2014handbook}, double the number of visitors the website sees in the second scenario.

\paragraph{Data collection decoupled from experiment hypotheses}
Traditionally, an experiment dataset is strongly dependent on the experiment's hypothesis and thus generally not reusable to evaluate other hypotheses. %\footnote{Not to be confused with the \emph{external validity} of an experiment, which refers to the validity of one extrapolating the \emph{results/conclusion} of one experiment to another.} 
This is because experimenters only collect the minimum necessary data to evaluate the hypothesis, not more on time and resource cost grounds. As mentioned above, the Web has largely eliminated the time and resource burdens, encouraging one to collect data that would otherwise not be collected. Referring to the  e-commerce website example (as illustrated in Figure~\ref{fig:intro_exp_abtestillustration_freedelivery}), it is now common for digital organisations to track and record all the elements on the web page shown to visitors. These may include whether a banner appeared on the web page, and if so, whether it is a ``free delivery'' banner or something else.
Such data collection will still happen even when we are not running any experiments or intend to run a completely different experiment, effectively decoupling it from specific experiment hypotheses.
Experimenters may also utilise the extra data collected -- be it experimental/observational or acting as a covariate/response -- to improve estimates on the effect of the treatments we are evaluating.

==> frontmatter/dedication.tex <==
% \cleardoublepage

\begin{dedication}
  Dedication here.
\end{dedication}
